Local Enumeration: The Not-All-Equal Case

Gurumukhani et al. (CCC'24) proposed the local enumeration problem Enum(k, t) as an approach to break the Super Strong Exponential Time Hypothesis (SSETH): for a natural number $k$ and a parameter $t$, given an $n$-variate $k$-CNF with no satisfying assignment of Hamming weight less than $t(n)$, enumerate all satisfying assignments of Hamming weight exactly $t(n)$. Furthermore, they gave a randomized algorithm for Enum(k, t) and employed new ideas to analyze the first non-trivial case, namely $k = 3$. In particular, they solved Enum(3, n/2) in expected $1.598^n$ time. A simple construction shows a lower bound of $6^{\frac{n}{4}} \approx 1.565^n$. In this paper, we show that to break SSETH, it is sufficient to consider a simpler local enumeration problem NAE-Enum(k, t): for a natural number $k$ and a parameter $t$, given an $n$-variate $k$-CNF with no satisfying assignment of Hamming weight less than $t(n)$, enumerate all Not-All-Equal (NAE) solutions of Hamming weight exactly $t(n)$, i.e., those that satisfy and falsify some literal in every clause. We refine the algorithm of Gurumukhani et al. and show that it optimally solves NAE-Enum(3, n/2), namely, in expected time $poly(n) \cdot 6^{\frac{n}{4}}$.

==> setup/preamble.tex <==
\RequirePackage{mathtools,amsmath,amsthm,amssymb,amscd,amsfonts}
\RequirePackage{scalefnt}
\usepackage[T1]{fontenc}
\usepackage{slantsc}
\usepackage[utf8]{inputenc}
\RequirePackage[dvipsnames]{xcolor}
\usepackage{lmodern}
\usepackage{bbm}
\usepackage{comment}
\usepackage[mathscr]{euscript}
\RequirePackage[letterpaper,top=1in,bottom=1in,left=1in,right=1in]{geometry}
\RequirePackage{tikz,pgf}
\RequirePackage{graphicx}
\RequirePackage[classfont=bold,langfont=roman,funcfont=typewriter,full,classfont=bold,langfont=caps,funcfont=typewriter,full]{complexity}
\RequirePackage{algpseudocode,algorithm,algorithmicx}
\usepackage{todonotes}
\usepackage[colorlinks=true,citecolor=blue,linkcolor=blue]{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}

\usepackage[nameinlink, noabbrev, capitalize]{cleveref}
\usepackage[inline]{enumitem}

\usepackage[
backend=biber,
style=alphabetic,
sorting=nyt,
maxnames=8,
maxalphanames=8,
% sortcites,
backref=true,
url=false
]{biblatex}

\usepackage{subfiles}

\AtBeginDocument{%
  \DeclareFontShape{T1}{lmr}{m}{scit}{<->ssub*lmr/m/scsl}{}%
}



%Algorithmicx package
%\algrenewcommand\algorithmicrequire{\textbf{Input:}}
%\algrenewcommand\algorithmicensure{\textbf{Output:}}
%\RequirePackage[12tabu, orthodox]{nag}
%\RequirePackage{caption}
%\RequirePackage{siunitx}
%\RequirePackage{verbatim}
%\RequirePackage{enumerate}
%\RequirePackage{fancyvrb}
%\RequirePackage{float}
%\usepackage{mathrsfs} %formal math script font
%\usepackage{bbm}
%\RequirePackage{braket}
%\usepackage{natbib}
%\usepackage{bibentry}
%\nobibliography*

